Deciding definability in FO2(<h,<v) on trees

We provide a decidable characterization of regular forest languages definable in FO2(<h,<v). By FO2(<h,<v) we refer to the two variable fragment of first order logic built from the descendant relation and the following sibling relation. In terms of expressive power it corresponds to a fragment of the navigational core of XPath that contains modalities for going up to some ancestor, down to some descendant, left to some preceding sibling, and right to some following sibling. We also show that our techniques can be applied to other two variable first-order logics having exactly the same vertical modalities as FO2(<h,<v) but having different horizontal modalities.

==> main-part.tex <==
For this section we fix a regular forest language $L$ recognized by a
morphism $\alpha: \A^\mydelta \rightarrow (H,V)$ into a 
finite forest algebra $(H,V)$. Assume that $H$ and $V$ satisfy
Identities~\eqref{eqh} and~\eqref{eqv} and that the leaf completion of
$\alpha$ is closed under saturation. We prove that any language
recognized by $\alpha$, including $L$, is definable in \FOd,
concluding the proof of Theorem~\ref{th-efmax}.

Recall that given a forest $s$ (a context $p$) we refer to its image
by $\alpha$ as the \emph{forest type} of $s$ (the \emph{context type}
of $p$). In view of Lemma~\ref{lem:leafsurj}, we assume without loss
of generality that $\alpha$ itself is leaf surjective and closed under
saturation. By definition, this implies in particular that for each $h
\in H$ there exists a tree consisting of a single node whose forest
type is $h$.

As mentioned earlier, we will often manipulate \shals modulo \mequivk
for some fixed integer $k$. We start by defining a suitable $k$. Given
a \shal $q$ and a forest $s$ we denote by $q[\bar s]$ the forest
constructed from $q$ by placing $s$ at each port of $q$.

\begin{lemma} \label{lem-choicek}
There exists a number $k'$ such that for all  $k\geq k'$, for all
\shals $p \mequivk p'$ and for all forests $s$, $p[\bar s]$ and
$p'[\bar s]$ have the same forest type.
\end{lemma}

\begin{proof}
This is a consequence of Theorem~\ref{thm-word-fod} and the fact that
$H$ satisfies Identity~\eqref{eqh}. Consider strings over $H$ as
alphabet and the natural morphism $\beta : H^{+} \rightarrow H$. Since
$H$ satisfies Identity~\eqref{eqh}, it follows from
Theorem~\ref{thm-word-fod} that for every $h \in H$, $\beta^{-1}(h)$
is definable using a formula of $\varphi_h$ of \FOdw. We choose $k'$
as the maximal rank of all these formulas.

Let $k \geq k'$ and take $p \mequivk p'$ and $s$ some forest. Let
$t_1,\dots,t_n$ be the sequence of trees occurring in $p[\bar s]$ and
$t'_1,\dots,t'_{n'}$ be the sequence of trees 
occurring in $p'[\bar s]$.  For all $i$ let $h_i = \alpha(t_i)$ and
$h'_i=\alpha(t'_i)$. As $p\mequiv{k} p'$ the strings $h_1\dots h_n$
and $h'_1\dots h'_{n'}$ satisfy the same formulas of \FOdw of rank
$k'$ over the alphabet $H$.  Let $h = \beta(h_1\dots h_n)$, by our
choice of $k'$ it follows that $h'_1\dots h'_{n'} \models
\varphi_h$. Hence $\beta(h_1\dots h_n) = h = \beta(h'_1\dots
h'_{n'})$. Therefore $\alpha(p[\bar s])=\alpha(p'[\bar s])$.
\end{proof} 

As $\alpha$ is closed under saturation, there is an integer $k''$ such
that $\alpha$ is closed under $k''$-saturation. We set $k$ as the
maximum of $k'$ as given by Lemma~\ref{lem-choicek} and
$k''$. By Lemma~\ref{lem-sat-k}, $\alpha$ remains closed
under $k$-saturation. Recall that a set $P$ of \shals is $k$-definable if
it is a union of equivalence classes of $\mequivk$.

Recall that $V^{\one}$ is the monoid obtained from $V$ by adding a
neutral element $\one_V$.
For each $h \in H$, $v \in V^{\one}$ and each 
set $P$ of \shals let
\[
L^P_{v,h}=\{t ~|~ v\alpha(t)=h \text{ and $t$ is $P$-valid}\}
\]
Our goal in this section is to show that:

\begin{proposition}\label{main-prop}
For all $h \in H$, all $v\in V^{\one}$ and all 
%\kdef
sets $P$ of \shals, there exists a language definable in \FOd that
agrees with $L^P_{v,h}$ on $P$-valid forests.
\end{proposition}

Theorem~\ref{th-efmax} is a direct consequence of
Proposition~\ref{main-prop}. Let $L'$ be the union of all definable languages
resulting from applying Proposition~\ref{main-prop} to all $L^P_{v,h}$
where $h \in \alpha(L)$, $v = 1_V$ and $P$ is the set of all \shals. By
definition $L'$ is definable in \FOd and agrees with $L$ on all $P$-valid
forests. Hence $L = L' \cup \{a \in A \mid a \in L\}$ which is
definable in \FOd.

The remainder of this section is devoted to the proof of
Proposition~\ref{main-prop}. Assume that $v,h$ and $P$ are fixed as in the
statement of the proposition, we prove that there exists a definable language
that agrees on $L_{v,h}^P$ on $P$-valid forests. We begin by considering the
special case when $P$ is not branching (i.e. contains only \shals of arity $0$
or $1$). In that case we conclude directly by
applying Theorem~\ref{thm-word-fod}.

\subsection{Special Case: $P$ is not branching} In this case we treat
our forests as strings and use the known results on strings. Since all
\shals in $P$ have arity $0$ or $1$, any $P$-valid forest $t$ is of
the form:  
\[
c_{1} \cdots c_{k}s 
\]
where $k$ is possibly $0$ and the $c_{1},\cdots,c_{k}$ are $P$-valid
\shals of arity $1$ and $s$ a $P$-valid \shal of arity $0$. For each
$u\in V^{\one}$ and $g\in H$, consider the languages:
\begin{equation*}
\begin{split}
M_{u,g} = \set{t ~~~|~~~  t=c_{1} \cdots c_{k} s \text{ is } P\text{-valid},
\alpha(c_{1}\cdots c_{k}) = u,  \text{ and } \alpha(s)=g}
\end{split}
\end{equation*}
Notice that $L^P_{v,h}$ is the union of those languages where
$vug=h$. We show that for any $u$ and $g$, there exists a language definable in
\FOd that agrees with $M_{u,g}$ on $P$-valid forests. This will conclude this case.

By definition \shals of arity $1$ are contexts. Let $\set{v_{1},...,v_{n}}$ be
the context types that are images of \shals of arity $1$ in $P$. 

Let $P'$ be the set of \shals from $P$ of arity 1. Let $p,p' \in P'$,
by Lemma~\ref{lem-choicek} if $p \mequivk p'$ for all
forests $s$, $p[s]$ and $p'[s]$ have the same forest type. Hence, $p$
and $p'$ have the same context type. This means that for all $v_i$ the
set of \shals of context type $v_i$ is $k$-definable. Therefore, by
Claim~\ref{lemma-p-valid}, there is a formula $\theta_{v_i}(x)$ of
\FOd testing whether the \shal of $x$ has $v_i$ as forest type.

Let $\Gamma = \set{d_{1},...,d_{n}}$ be an alphabet and define a morphism
$\beta : \Gamma^{*} \rightarrow V$ by $\beta(d_{i}) = v_{i}$. Since $V$
satisfies Identity~(\ref{eqv}), for each $u \in V$ there is a \FOdw formula
$\varphi_{u}$ such that the strings of $\Gamma^{*}$ satisfying $\varphi_{u}$
are the strings of type $u$ under $\beta$. From $\varphi_{u}$ we construct a
formula $\Psi_{u}$ of \FOd defining all $P'$-valid contexts having $u$ as
context type. This is done by replacing in $\varphi_u$ all atomic formulas
$P_{d_{i}}(x)$ with $\theta_{v_i}(x)$. We can also easily define in \FOd the
set of \shals of arity $0$ such that $\alpha(s)=g$. After combining this last
formula with $\Psi_u$ we get the desired language definable in \FOd and
agreeing with $M_{u,g}$ on $P$-valid forests.

\medskip

In the remainder of the proof we assume that $P$ is branching, i.e. it
contains one \shal of arity at least~2. Recall, that by
Claim~\ref{claim-maximal}, it follows that there exists a unique
maximal $P$-reachable class $H_P$. The rest of the proof is by
induction on three parameters that we now define.

\subsection{Induction Parameters} The first and most important of our
induction parameters is the size of the set of $P$-valid forest
types. We denote this set by $X$. Observe that by definition $H_P
\subseteq X$.

\smallskip

Our second parameter is an index defined on sets $P$ of \shals. During
the proof we will construct from $P$ new sets $P'$ by replacing some
of their port-nodes with \Xnodes. Our definition ensures that the
index of $P'$ will be smaller than the index of $P$, hence guarantees
termination of the induction. It is based on following preorder on
\shals called simulation modulo~$X$.

Given two \shals $p$ and $p'$, we say that \emph{$p$ simulates $p'$
  modulo $X$} if $p'$ is obtained from $p$ by replacing some of its
port-nodes $b(\hole)$ by an \Xnode $b(a)$ with the same inner
label. Observe that simulation modulo $X$ is a partial order.


For each \shal $p$ its \emph{$X$-number} is the number of non
$\pequiv{k+2}^X$-equivalent \shals $q$ (not necessarily in $P$) that
can be simulated modulo $X$ by $p$. For each set $P$ of \shals the
\emph{$n$-index of $P$} is the number of non $\pequiv{k+2}^X$-equivalent
\shals $p \in P$ of $X$-number $n$. Our second induction parameter,
called the \emph{index of $P$}, is the sequence of its $n$-indexes
ordered by decreasing $n$.



\smallskip

The third parameter is based on $v$. Consider the preorder on context
types defined by the quotient of the $P$-reachability relation by the
$P$-equivalence relation. The \emph{$P$-depth} of a context type $v$
is the maximal length of a path in this preorder from the empty context~to~$v$.

\smallskip

We prove Proposition~\ref{main-prop} by induction on the following
three parameters, given below in their order of importance:

\begin{center}
\begin{enumerate}[(i)]
 \item $|X|$
 \item the index of $P$
 \item the $P$-depth of $v$
 \end{enumerate}
\end{center}

We distinguish three cases: a base case and two cases in which we will 
use antichain composition and induction. We say that a context type
$u$ \emph{$P$-preserves} $v$ if $v$ is $P$-reachable from $vu$. A
context $c$ \emph{$P$-preserves} $v$ if its context-type $P$-preserves
$v$.

\subsection{Base Case: $P$ is reduced and $v$ is $P$-preserved by a
  \saturated{(P,k)} context $\Delta$}  We use saturation to prove that
$v$ is constant over the set $X = H_P$ of $P$-valid forest types,
i.e. for any $P$-valid $h_1,h_2 \in H$, $vh_1 = vh_2$. Since all forests in $L^P_{v,h}$
are $P$-valid, it follows that $L^P_{v,h}$ is either empty or the
language of all $P$-valid forests. The desired definable language is
therefore either the empty language of the language of all forests.

Since $\Delta$ $P$-preserves $v$, there exists a $P$-valid context $c$
such that $v\alpha(\Delta c) = v$. It follows that $v = v
\alpha(\Delta c)^{\omega}$. Moreover, observe that since $\Delta$ is
$P$-saturated and $c$ is $P$-valid, $\Delta c$ is $P$-saturated as
well. It then follows from saturation that

\[
vh_1 = v \alpha(\Delta c)^{\omega}h_1 = v \alpha(\Delta c)^{\omega}h_2
= vh_2
\]

This terminates the proof of the base case. We now consider two cases
in which we conclude by induction.

\subsection{Case 1: $P$ is not reduced, Bottom-Up Induction.}
\input{bottomup}

\subsection{Case 2: $P$ is reduced but there exists no
  \saturated{(P,k)} context $\Delta$ that $P$-preserves $v$, Top-Down
  Induction}

\input{topdown}

%%% Local Variables: 
%%% TeX-PDF-mode: t
%%% TeX-master: "main"
%%% ispell-local-dictionary: "american"
%%% End:  



